AniGS: Animatable Gaussian Avatar from a Single Image with Inconsistent Gaussian Reconstruction

Generating animatable human avatars from a single image is essential for various digital human modeling applications. Existing 3D reconstruction methods often struggle to capture fine details in animatable models, while generative approaches for controllable animation, though avoiding explicit 3D modeling, suffer from viewpoint inconsistencies in extreme poses and computational inefficiencies. In this paper, we address these challenges by leveraging the power of generative models to produce detailed multi-view canonical pose images, which help resolve ambiguities in animatable human reconstruction. We then propose a robust method for 3D reconstruction of inconsistent images, enabling real-time rendering during inference. Specifically, we adapt a transformer-based video generation model to generate multi-view canonical pose images and normal maps, pretraining on a large-scale video dataset to improve generalization. To handle view inconsistencies, we recast the reconstruction problem as a 4D task and introduce an efficient 3D modeling approach using 4D Gaussian Splatting. Experiments demonstrate that our method achieves photorealistic, real-time animation of 3D human avatars from in-the-wild images, showcasing its effectiveness and generalization capability.

==> tables/equations.tex <==
\newcommand{\normal}{\boldsymbol{n}}
\newcommand{\point}{\boldsymbol{x}}

%\resizebox{0.48\textwidth}{!}{
    %\large
\renewcommand{\arraystretch}{1.3}
    \begin{tabular}{llll}
        \toprule
        Notation & Example\\
        \midrule
         Fraction &  $\frac{1}{a}$ \\
         Max & $\max (a, 0 )$ \\
         Dimension & $\boldsymbol{x} \in \mathbb{R}^3$ \\
         Argmax  & $\mathop{\arg\max}_{a} f(ax)$ \\
         cos & $\cos(x)$ \\
         Hat/tilde & $\hat{\boldsymbol{x}}, \tilde{\boldsymbol{x}}$ \\
         Tensor operation & $\otimes$, \quad $\circ$, \quad $\odot$ \\ 
         Sum & $\sum_{i=1}^{N} x_i$ \\
         Approximation & $f(x) \approx g(x)$ \\
         Around & $\sim$100 \\
         Product & $\prod_{i=1}^{N} x_i$ \\
         Integral & $\int_{-\infty}^{+\infty} x_i$ \\
         Gradient & $\boldsymbol{n}(n) = \nabla o(\boldsymbol{x})/\|\nabla o(\boldsymbol{x})\|_2$ \\
         Parallel & $\mathcal{L} = \sum \| x_i - \hat{x}_i \|^2_2$ \\
         Set & $\{I_i | i=1,\dots, N \}$ \\
        \bottomrule
    \end{tabular}
%    }



==> tables/greek_letters.tex <==
    \resizebox{0.48\textwidth}{!}{
    \large
    \begin{tabular}{clclclclc}
        \toprule
        Symbol & \LaTeX  & Symbol & \LaTeX & Symbol & \LaTeX\\
        \midrule
$\alpha  $ & \textbackslash alpha   & $\kappa $ & \textbackslash kappa  & $\psi    $  & \textbackslash psi    \\
$\beta   $ & \textbackslash beta    & $\lambda$ & \textbackslash lambda & $\rho    $  & \textbackslash rho    \\
$\chi    $ & \textbackslash chi     & $\mu    $ & \textbackslash mu     & $\sigma  $  & \textbackslash sigma  \\
$\delta  $ & \textbackslash delta   & $\nu    $ & \textbackslash nu     & $\tau    $  & \textbackslash tau    \\
$\epsilon$ & \textbackslash epsilon & $ o     $ & \textbackslash o      & $\theta  $  & \textbackslash theta  \\
$\eta    $ & \textbackslash eta     & $\omega $ & \textbackslash omega  & $\upsilon$  & \textbackslash upsilon\\
$\gamma  $ & \textbackslash gamma   & $\phi   $ & \textbackslash phi    & $\xi     $  & \textbackslash xi     \\
$\iota   $ & \textbackslash iota    & $\pi    $ & \textbackslash pi     & $\zeta   $  & \textbackslash zeta   \\
\midrule
$ \digamma   $ & \textbackslash digamma    & $ \Delta $ & \textbackslash digamma    & $ \Theta   $  & \textbackslash Theta  \\
$ \varepsilon$ & \textbackslash varepsilon & $ \Gamma $ & \textbackslash varepsilon & $ \Upsilon $  & \textbackslash Upsilon\\
$ \varkappa  $ & \textbackslash varkappa   & $ \Lambda$ & \textbackslash varkappa   & $ \Xi      $  & \textbackslash Xi     \\
$ \varphi    $ & \textbackslash varphi     & $ \Omega $ & \textbackslash varphi     &               &         \\
$ \varpi     $ & \textbackslash varpi      & $ \Phi   $ & \textbackslash varpi      & $ \aleph   $  & \textbackslash aleph  \\
$ \varrho    $ & \textbackslash varrho     & $ \Pi    $ & \textbackslash varrho     & $ \beth    $  & \textbackslash beth   \\
$ \varsigma  $ & \textbackslash varsigma   & $ \Psi   $ & \textbackslash varsigma   & $ \daleth  $  & \textbackslash daleth \\
$ \vartheta  $ & \textbackslash vartheta   & $ \Sigma $ & \textbackslash vartheta   & $ \gimel   $  & \textbackslash gimel  \\
        \bottomrule
    \end{tabular}
    }



==> tables/two_subtables.tex <==
\newcommand{\PSNRT}{PSNR\xspace}
\newcommand{\VQM}{HDR-VQM\xspace}
\newcommand{\VDP}{HDR-VDP2\xspace}
\newcommand{\LowExposure}{Low-Exposure\xspace}
\newcommand{\MiddleExposure}{Middle-Exposure\xspace}
\newcommand{\HighExposure}{High-Exposure\xspace}
\newcommand{\AllExposure}{All-Exposure\xspace}

\makebox[\textwidth]{\small (a) Results on dataset A.} 
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{2}{c}|*{2}{c}|*{3}{c}||*{2}{c}|*{2}{c}|*{2}{c}|*{3}{c}}
    \toprule
    & \multicolumn{7}{c||}{2-Exposure} & \multicolumn{9}{c}{3-Exposure} \\
    & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c||}{\AllExposure} & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\MiddleExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c}{\AllExposure} \\
    Method & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \VQM & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \PSNRT & \VDP & \VQM \\
    \midrule
    Method A & \Scnd{40.00} & 73.70 & \Scnd{40.04} & \Scnd{70.08} & \Scnd{40.02} & 71.89 & \Scnd{76.22} 
                  & \Scnd{39.61} & 73.24 & \Frst{39.67} & \Frst{73.24} & \Frst{40.01} & 67.90 & \Frst{39.77} & 70.37 & 79.55 \\
    Method B      & 34.54 & 80.22 & 39.25 & 65.96 & 36.90 & 73.09 & 65.33 
                  & 36.51 & 77.78 & 37.45 & 69.79 & 39.02 & 64.57 & 37.66 & 70.71 & 70.13 \\
    Method C  & 39.79 & \Scnd{81.02} & 39.96 & 67.25 & 39.88 & \Scnd{74.13} & 73.84 
                  & 39.48 & \Scnd{78.13} & 38.43 & 70.08 & 39.60 & \Scnd{67.94} & 39.17 & \Scnd{72.05} & \Scnd{80.70} \\
    Ours          & \Frst{41.95} & \Frst{81.03} & \Frst{40.41} & \Frst{71.27} & \Frst{41.18} & \Frst{76.15} & \Frst{78.84}
                  & \Frst{40.00} & \Frst{78.66} & \Scnd{39.27} & \Scnd{73.10} & \Scnd{39.99} & \Frst{69.99} & \Scnd{39.75} & \Frst{73.92} & \Frst{82.87} \\
    \bottomrule
\end{tabular}
}

\vspace{0.5em}
\makebox[\textwidth]{\small (b) Results on dataset B.} 
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{2}{c}|*{2}{c}|*{3}{c}||*{2}{c}|*{2}{c}|*{2}{c}|*{3}{c}}
    \toprule
    & \multicolumn{7}{c||}{2-Exposure} & \multicolumn{9}{c}{3-Exposure} \\
    & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c||}{\AllExposure} & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\MiddleExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c}{\AllExposure} \\
    Method & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \VQM & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \PSNRT & \VDP & \VQM \\
    \midrule
    Method A & 37.73 & 74.05 & 45.71 & 66.67 & 41.72 & 70.36 & 85.33 
                  & 37.53 & 72.03 & 36.38 & 65.37 & 34.73 & 62.24 & 36.21 & 66.55 & 84.43 \\
    Method B      & 36.41 & 85.68 & \Scnd{49.89} & \Scnd{69.90} & 43.15 & 77.79 & 78.92 
                  & 36.43 & 77.74 & 39.80 & \Scnd{67.88} & \Scnd{43.03} & \Scnd{64.74} & 39.75 & \Scnd{70.12} & 87.93 \\
    Method C  & \Scnd{39.94} & \Scnd{86.77} & 49.49 & 69.04 & \Scnd{44.72} & \Scnd{77.91} & \Scnd{87.16} 
                  & \Scnd{38.34} & \Scnd{78.04} & \Scnd{41.21} & 66.07 & 42.66 & 64.01 & \Scnd{40.74} & 69.37 & \Scnd{89.36}\\
    Ours          & \Frst{40.83} & \Frst{86.84} & \Frst{50.10} & \Frst{71.33} & \Frst{45.46} & \Frst{79.09} & \Frst{87.40} 
                  & \Frst{38.77} & \Frst{78.11} & \Frst{41.47} & \Frst{68.49} & \Frst{43.24} & \Frst{65.08} & \Frst{41.16} & \Frst{70.56} & \Frst{89.56}\\
    \bottomrule
\end{tabular}
}

